WOMD-LiDAR: Raw Sensor Dataset Benchmark for Motion Forecasting

Widely adopted motion forecasting datasets substitute the observed sensory inputs with higher-level abstractions such as 3D boxes and polylines. These sparse shapes are inferred through annotating the original scenes with perception systems' predictions. Such intermediate representations tie the quality of the motion forecasting models to the performance of computer vision models. Moreover, the human-designed explicit interfaces between perception and motion forecasting typically pass only a subset of the semantic information present in the original sensory input. To study the effect of these modular approaches, design new paradigms that mitigate these limitations, and accelerate the development of end-to-end motion forecasting models, we augment the Waymo Open Motion Dataset (WOMD) with large-scale, high-quality, diverse LiDAR data for the motion forecasting task. The new augmented dataset WOMD-LiDAR consists of over 100,000 scenes that each spans 20 seconds, consisting of well-synchronized and calibrated high quality LiDAR point clouds captured across a range of urban and suburban geographies (https://waymo.com/open/data/motion/). Compared to Waymo Open Dataset (WOD), WOMD-LiDAR dataset contains 100x more scenes. Furthermore, we integrate the LiDAR data into the motion forecasting model training and provide a strong baseline. Experiments show that the LiDAR data brings improvement in the motion forecasting task. We hope that WOMD-LiDAR will provide new opportunities for boosting end-to-end motion forecasting models.

==> figures/fig2_sync_dist.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.8\linewidth]{figures/images/time_diff_hist.pdf}
\end{center}
\vspace{-6mm}
  \caption{Synchronization difference in microseconds ($\mu$s) between {\lidar} data and machine generated labels of \revonly{{\dbname}}\arxivonly{WOMD~\cite{ettinger2021large}}. Most time differences are within +/- 50 $\mu$s.}
\label{fig:sync_dist}
\end{figure}

==> figures/fig3_lidar_viz.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{figures/images/lidar_viz.png}
\end{center}
\vspace{-2mm}
  \caption{Visualization of LiDAR point cloud with auto-labeled boxes in one scene from {\dbname}.}
\label{fig:lidar_viz}
\end{figure}

==> figures/fig5_drop_future_lidar.tex <==
\begin{figure}[!hbt]
\begin{center}
\includegraphics[width=1.0\linewidth]{figures/images/drop_future_lidar.pdf}
\end{center}
\vspace{-2mm}
  \caption{{\lidar} data of {\dbname} in future steps is not necessary for training a motion forecasting model. The first 1 second (11 steps) contains past and current data where {\lidar} is needed as input for a motion forecasting model. The rest of 8 second (80 steps) in the scene contains future steps' data, where only ground truth is needed to calculate loss and metrics.
  }
\label{fig:drop_future_lidar}
\end{figure}

==> figures/fig7_det_dist.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.70\linewidth]{figures/images/hist_det.pdf}

\caption{Distribution of the number of detected objects by {\swf} in each frame of {\dbname}.}
\label{fig:det_dist}
\end{figure}

==> figures/fig9_swformer_det.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{figures/images/swformer_det_viz.pdf}


\caption{Visualization of {\swf} detection results on one of {\dbname} scenes. The detected boxes of different objects form continuous trajectories across different time steps.}
\label{fig:swformer_det}
\end{figure}


==> tables/dummy_table1.tex <==
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\

==> tables/supp_tab_test_set.tex <==
\begin{table*}[b]
\begin{center}
\small
\begin{tabular}{@{}cc|ccc|ccc|ccc@{}}
\toprule
\multirow{2}{*}{Set} &
  \multirow{2}{*}{Model} &
  \multicolumn{3}{c|}{Vehicle} &
  \multicolumn{3}{c|}{Pedestrian} &
  \multicolumn{3}{c}{Cyclist} \\
 &
  &
  minADE $\downarrow$ &
  MR $\downarrow$ &
  mAP $\uparrow$ &
  minADE $\downarrow$ &
  MR $\downarrow$ &
  mAP $\uparrow$ &
  minADE $\downarrow$ &
  MR $\downarrow$ &
  mAP $\uparrow$ \\ \midrule
% \multicolumn{1}{l}{} &
%   LSTM~\cite{ettinger2021large} &
%   \multicolumn{1}{c}{1.34} & 
%   \multicolumn{1}{c}{0.25} & 
%   \multicolumn{1}{c|}{0.23} & 
%   \multicolumn{1}{c}{0.63} &
%   \multicolumn{1}{c}{0.13} &
%   \multicolumn{1}{c|}{0.23} &
%   \multicolumn{1}{c}{1.26} &
%   \multicolumn{1}{c}{0.29} &
%   \multicolumn{1}{c}{0.21} \\ \cmidrule(l){2-11} 
% \begin{tabular}[c]{@{}c@{}}Standard\\ Validation\end{tabular} &
%   Wayformer~\cite{nayakanti2022wayformer}
%   & 1.10
%   & 0.18
%   & 0.35
%   & 0.54
%   & 0.11
%   & 0.35
%   & 1.08
%   & 0.22
%   & \textbf{0.29}
%   \\ \cmidrule(l){2-11} 
%  &
%   \begin{tabular}[c]{@{}c@{}}Wayformer\\ + LiDAR\end{tabular} 
%   & \textbf{1.09}
%   & \textbf{0.17}
%   & \textbf{0.37}
%   & \textbf{0.54}
%   & \textbf{0.10}
%   & \textbf{0.37}
%   & \textbf{1.06}
%   & \textbf{0.21}
%   & 0.28
%   \\ 
% \midrule \midrule
\multicolumn{1}{l}{} &
  LSTM~\cite{ettinger2021large} &
  \multicolumn{1}{c}{1.34} & 
  \multicolumn{1}{c}{0.24} & 
  \multicolumn{1}{c|}{0.24} & 
  \multicolumn{1}{c}{0.64} &
  \multicolumn{1}{c}{0.13} &
  \multicolumn{1}{c|}{0.22} &
  \multicolumn{1}{c}{1.29} &
  \multicolumn{1}{c}{0.28} &
  \multicolumn{1}{c}{0.20} \\ \cmidrule(l){2-11} 
\begin{tabular}[c]{@{}c@{}}Standard\\ Test\end{tabular} &
  Wayformer~\cite{nayakanti2022wayformer}
  & 1.07
  & 0.17
  & 0.37
  & 0.54
  & 0.10
  & 0.37
  & 1.06 
  & 0.20
  & 0.30
  \\ \cmidrule(l){2-11} 
 &
  \begin{tabular}[c]{@{}c@{}}Wayformer\\ + LiDAR\end{tabular} 
  & 
  & 
  & 
  & 
  &
  &
  &
  &
  &
   \\ \bottomrule
\end{tabular}
\end{center}
\caption{\txbu{Marginal} \textbf{metrics on the} \txbu{standard} \textbf{validation set}. All metrics computed at 8s. We implement and compare our own WOMD~\cite{ettinger2021large} baseline, {\wf}~\cite{nayakanti2022wayformer} and {\wf} trained with {\lidar} data on the {\dbname} standard motion forecasting track.
}
\label{tab:supp_exp_res_standard}
\end{table*}
